Fast Density-Peaks Clustering: Multicore-based Parallelization Approach

Clustering multi-dimensional points is a fundamental task in many fields, and density-based clustering supports many applications as it can discover clusters of arbitrary shapes. This paper addresses the problem of Density-Peaks Clustering (DPC), a recently proposed density-based clustering framework. Although DPC already has many applications, its straightforward implementation incurs a quadratic time computation to the number of points in a given dataset, thereby does not scale to large datasets. To enable DPC on large datasets, we propose efficient algorithms for DPC. Specifically, we propose an exact algorithm, Ex-DPC, and two approximation algorithms, Approx-DPC and S-Approx-DPC. Under a reasonable assumption about a DPC parameter, our algorithms are sub-quadratic, i.e., break the quadratic barrier. Besides, Approx-DPC does not require any additional parameters and can return the same cluster centers as those of Ex-DPC, rendering an accurate clustering result. S-Approx-DPC requires an approximation parameter but can speed up its computational efficiency. We further present that their efficiencies can be accelerated by leveraging multicore processing. We conduct extensive experiments using synthetic and real datasets, and our experimental results demonstrate that our algorithms are efficient, scalable, and accurate.

==> Algorithm/approx-dpc.tex <==
\begin{algorithm}[!t]
	\caption{Approx-DPC}	\label{algo_approx-dpc}
	\DontPrintSemicolon
    {\small
        \KwIn {$P$ (a point set), $d_{cut}$, $\mathcal{K}$ (a $k$d-tree)}
		\vspace{1.0mm}
        /* Grid building */\;
        $G \leftarrow \varnothing$\;									\label{approx-dpc_line_grid_b}
        \For {each $p_{i} \in P$}{
        	$j \leftarrow$ key of the cell where $p_{i}$ is mapped\;
            \If {$c_{j} \notin G$} {
            	$G \leftarrow G \cup \{c_{j}\}$
            }
            $P(c_{j}) \leftarrow P(c_{j}) \cup \{p_{i}\}$				\label{approx-dpc_line_grid_e}
        }
        \vspace{1.0mm}
		/* Local density computation */\;
		\For {each $c \in G$}{											\label{approx-dpc_line_ld_b}
        	$cp \leftarrow$ the center point of $c$\;					\label{approx-dpc_line_joint_b}
            $r \leftarrow \max_{p \in P(c)}dist(cp,p)$\;
            $R(cp,d_{cut} + r) \leftarrow$ \textsc{Range-Search}$(cp, d_{cut} + r,\mathcal{K})$\;
            \For {each $p_{i} \in P(c)$}{
            	\For {each $p_{j} \in P(c)$ such that $i \neq j$}{
                	\If {$dist(p_{i},p_{j}) < d_{cut}$}{
                    	$\rho_{i} \leftarrow \rho_{i} + 1$				\label{approx-dpc_line_joint_e}
                    }
                }
                Update $p^{*}(c)$, $\min_{P(c)}\rho$ and $N(c)$			\label{approx-dpc_line_ld_e}
            }
        }
        \vspace{1.0mm}
        /* Approximate dependent point computation */\;
        \For {each $c \in G$}{																\label{approx-dpc_line_adp_b}
        	\For {each $p_{i} \in P(c)$}{
            	\eIf {$p_{i} \neq p^{*}(c)$}{
                	$q_{i} \leftarrow p^{*}(c)$, $\delta_{i} \leftarrow d_{cut}$
                }{
                	\For {each $c' \in N(c)$}{
                    	\If {$\min_{P(c')}\rho > \rho_{i}$}{
                        	$q_{i} \leftarrow p^{*}(c')$, $\delta_{i} \leftarrow d_{cut}$	\label{approx-dpc_line_adp_e}
                            \textbf{break}
                        }
                    }
                }
            }
        }
        \vspace{1.0mm}
        /* Exact dependent point computation */\;
        Sort $P$ in ascending order of local density\;										\label{approx-dpc_line_edp_b}
        Divide $P$ into $s$ disjoint subsets $P_{1}$, ..., $P_{s}$\;
        \For {each $i \in [1,s]$}{
        	Build a $k$d-tree $\mathcal{K}_{i}$ of $P_{i}$
        }
        $P' \leftarrow$ a set of points whose dependent points have not been decided\;
        \For {each $p_{i} \in P'$}{
        	\For {each $j \in [1,s]$}{
        		\Case {$\min_{p \in P_{j}}\rho > \rho_{i}$}{
            		$q_{i} \leftarrow$ \textsc{NN-Search}$(p_{i},\mathcal{K}_{j})$\;					\label{approx-dpc_line_nns}
                    Update $\delta_{i}$
            	}
                \Case {$\min_{p \in P_{j}}\rho < \rho_{i}$ and $\max_{p \in P_{i}}\rho < \rho_{i}$}{
                	Scan $P_{j}$ and update $q_{i}$ and $\delta_{i}$									\label{approx-dpc_line_edp_e}
                }
        	}
        }
	}
\end{algorithm}


==> Algorithm/ex-dpc.tex <==
\begin{algorithm}[!h]
	\caption{Ex-DPC}	\label{algo_ex-dpc}
	\DontPrintSemicolon
    {\small
        \KwIn {$P$ (a point set), $d_{cut}$, $\mathcal{K}$ (a $k$d-tree)}
		\vspace{1.0mm}
		/* local density computation */\;
		\For {each $p_{i} \in P$}{														\label{ex-dpc_line_ld_b}
        	$\rho_{i} \leftarrow$ \textsc{Range-Search}$(p_{i},d_{cut},\mathcal{K})$	\label{ex-dpc_line_ld_e}
        }
        \vspace{1.0mm}
        /* dependent point computation */\;
        $\mathcal{K} \leftarrow \varnothing$\;								\label{ex-dpc_line_dp_b}
        Sort $P$ in descending order of local density\;
        \For {each $p_{i} \in P$}{
        	$q_{i} \leftarrow$ \textsc{NN-Search}$(p_{i},\mathcal{K})$\;	\label{ex-dpc_line_nns}
            \textsc{Insert}$(p_{i},\mathcal{K})$							\label{ex-dpc_line_dp_e}
        }
	}
\end{algorithm}


==> Algorithm/s-approx-dpc.tex <==
\begin{algorithm}[!t]
	\caption{S-Approx-DPC}	\label{algo_s-approx-dpc}
	\DontPrintSemicolon
    {\small
        \KwIn {$P$ (a point set), $d_{cut}$, $\epsilon$, $\mathcal{K}$ (a $k$d-tree)}
		\vspace{1.0mm}
        /* Grid building */\;
        $G' \leftarrow \varnothing$\;														\label{sapprox-dpc_line_grid_b}
        \For {each $p_{i} \in P$}{
        	$j \leftarrow$ key of the cell where $p_{i}$ is mapped (based on $\epsilon$)\;
            \If {$c_{j} \notin G'$} {
            	$G' \leftarrow G' \cup \{c_{j}\}$
            }
            $P(c_{j}) \leftarrow P(c_{j}) \cup \{p_{i}\}$									\label{sapprox-dpc_line_grid_e}
        }
        \vspace{1.0mm}
		/* Local density comp. */\;
		\For {each $c \in G'$}{																\label{sapprox-dpc_line_ld_b}
        	$p \leftarrow$ a sampled point in $c$\;	\label{s-approx-dpc_line_sample}
            $R(p,d) \leftarrow$ \textsc{Range-Search}$(p,d_{cut},\mathcal{K})$\;
            $\rho_{i} \leftarrow |R(p,d)|$\;
            Update $N(c)$ from $R(p,d)$\;													\label{sapprox-dpc_line_ld_e}
        }
        \vspace{1.0mm}
        /* Approximate dependent point comp. (1st phase) */\;
        \For {each $c \in G'$}{																			\label{sapprox-dpc_line_dp1_b}
        	$p_{i} \leftarrow$ the sampled point in $c$ at line \ref{s-approx-dpc_line_sample}\;
            \For {each $p_{j} \in P(c)\backslash\{p_{i}\}$}{
            	$q_{j} \leftarrow p_{i}$, $\delta_{j} \leftarrow dist(p_{i},p_{j})$
            }
        	\For {each $c' \in N(c)$}{
            	$p_{j} \leftarrow$ the sampled point in $c'$ at line \ref{s-approx-dpc_line_sample}\;
            	\If {$\rho_{i} < \rho_{j}$}{
                	$q_{i} \leftarrow p_{j}$, $\delta_{i} \leftarrow dist(p_{i},p_{j})$\;
                    \textbf{break}																		\label{sapprox-dpc_line_dp1_e}
                }
            }
        }
        \vspace{1.0mm}
        /* Approximate dependent point comp. (2nd phase) */\;
        $P'_{pick} \leftarrow$ a set of sampled points whose dependent points have not been obtained in the first phase\;			\label{sapprox-dpc_line_dp2_b}
        Form temporal clusters based on the dependence relationships obtained in the first phase\;									\label{sapprox-dpc_line_dp2_cluster}
        \For {each $p_{i}$ that is the center of a temporal cluster $T_{i}$}{
        	$r_{i} \leftarrow \max_{p \in T_{i} dist(p_{i},p)}$																		\label{sapprox-dpc_line_dp2_r}
        }
        \For {each $p_{i} \in P'_{pick}$}{
        	$p' \leftarrow \argmin_{p_{j} \in P'_{pick}, \rho_{i} < \rho_{j}} dist(p_{i},p_{j})$\;
            Retrieve $q'_{i}$ from $T_{j}$ such that $dist(p_{i},p_{j}) - r_{j} \leq dist(p_{i},p')$ and $\rho_{i} < \rho_{j}$\;
            $\delta_{i} \leftarrow dist(p_{i},q'_{i})$																				\label{sapprox-dpc_line_dp2_e}
        }
	}
\end{algorithm}


==> Algorithm/straightforward.tex <==
\begin{algorithm}[!h]
	\caption{Straightforward algorithm}	\label{algo_scan}
	\DontPrintSemicolon
	{\small
        \KwIn {$P$ (a point set), $d_{cut}$}

		\vspace{1.0mm}
		/* local density computation */\;
		\For {each $p_{i} \in P$}{
        	\For {each $p_{j} \in P$ such that $i \neq j$}{
            	\If {$dist(p_{i},p_{j}) < d_{cut}$}{
                	$\rho_{i} \leftarrow \rho_{i} + 1$
                }
            }
        }
        
        \vspace{1.0mm}
        /* dependent point computation */\;
        Sort $P$ in descending order of local density\;
        \For {each $p_{i} \in P$}{
        	$q_{i} \leftarrow \varnothing$, $\delta_{i} \leftarrow \infty$\;
        	\For {each $p_{j} \in P$ such that $\rho_{i} < \rho_{j}$}{
            	\If {$dist(p_{i},p_{j}) < \delta_{i}$}{
                	$\delta_{i} \leftarrow dist(p_{i},p_{j})$, $q_{i} \leftarrow p_{j}$
        		}
            }
        }
	}
\end{algorithm}

